Wiser: Increasing Throughput in Payment Channel Networks with Transaction Aggregation

Payment channel networks (PCNs) are one of the most prominent solutions to the limited transaction throughput of blockchains. Nevertheless, PCNs suffer themselves from a throughput limitation due to the capital constraints of their channels. A similar dependence on high capital is also found in inter-bank payment settlements, where the so-called netting technique is used to mitigate liquidity demands. In this work, we alleviate this limitation by introducing the notion of transaction aggregation: instead of executing transactions sequentially through a PCN, we enable senders to aggregate multiple transactions and execute them simultaneously to benefit from several amounts that may "cancel out". Two direct advantages of our proposal is the decrease in intermediary fees paid by senders as well as the obfuscation of the transaction data from the intermediaries. We formulate the transaction aggregation as a computational problem, a generalization of the Bank Clearing Problem. We present a generic framework for the transaction aggregation execution, and thereafter we propose Wiser as an implementation of this framework in a specific hub-based setting. To overcome the NP-hardness of the transaction aggregation problem, in Wiser we propose a fixed-parameter linear algorithm for a special case of transaction aggregation as well as the Bank Clearing Problem. Wiser can also be seen as a modern variant of the Hawala money transfer system, as well as a decentralized implementation of the overseas remittance service of Wise.

==> indistinguishability.tex <==
%\section{Privacy definition}\label{sec:privacy}
Here we define the notion of privacy we wish to achieve during the entire course of our protocol, i.e. both the flow computation and execution phases. 
We want to enforce, firstly, that each uninvolved user should only learn that they are not involved in the protocol. 
Secondly, each involved user (whether client or hub) should only learn the flow output on each of the incident channels to the hubs.
We stress that the above two conditions imply value privacy: users will not know the flow (and thus the transaction amounts) along channels they are not a part of. 
Finally, we allow each involved user to learn the number of other involved users in the protocol \footnote{Ideally, involved users should not learn any information about the set of other involved users in the protocol. However, our proposed flow execution protocol requires the number of involved users to be known in advance. We are working on future work to bound the number of involved users each involved user needs to know.}. 

%We note that in the execution of our protocol, all hubs and involved users would know the set of other involved users. This is a result of our choice of an atomic transaction flow execution protocol. While this is not ideal, we believe that this is not too big of an issue as users who wish to participate in the protocol could generate fresh pseudonymous public keys each time. We leave reducing the number of involved users known to any user to future work. 
Our notion of privacy is based on the following indistinguishability game between an passive adversary $\mathcal{A}$ and a transaction aggregation and execution protocol $\Pi$ when run on the subgraph of users interested in participating in the protocol $G=(V,E)$:

\begin{itemize}
    \item $\mathcal{A}$ chooses a subset of users $V^{\mathcal{A}} \subset V$ to corrupt, i.e. $\mathcal{A}$ gains access to the transcripts of every corrupted user $v \in V^{\mathcal{A}}$. 
    $V^{\mathcal{A}}$ can consist solely of hubs, clients, or a mix of both.
    Let $G^{\mathcal{A}}$ be the subgraph created by taking the union of all corrupted nodes and their incident edges. 
    Additionally, if a hub node is in $V^{\mathcal{A}}$, we add all the other hubs in the network and all incident edges within the factory to $G^{\mathcal{A}}$.
    \item $\mathcal{A}$ chooses the following for $i \in \{0,1\}$: $\mathcal{A}$ creates a list of transactions tuples $\mathcal{T}^i = \{(x_j, s_j, r_j)\}_{j=1}^{n_i}$ where the $j$th transaction tuple consists of a transaction amount $x_j$, the vertex $s_j$ that requested the transaction, and the vertex $r_j$ that should receive the transaction. $n_i$ is the number of transaction tuples in the $i$th list.
    \item For every node and channel in $G^{\mathcal{A}}$, the following condition needs to hold: the resulting flow returned by $\Pi$ restricted to the subgraph $G^{\mathcal{A}}$ when run on $G$ and when given transaction tuple lists $\mathcal{T}^0$ and $\mathcal{T}^1$ has to be the same. 
    %Additionally, the internal state of the factory before and after running $\Pi$ should be the same when executed on inputs $\mathcal{T}^0$ and $\mathcal{T}^1$. 
    Additionally, the set of involved users as computed by $\Pi$ should be the same when given $\mathcal{T}^0$ or $\mathcal{T}^1$ as input. 
    %Each corrupted hub has to see the same number of transactions, transaction amounts as well as the senders and recipients of these transactions in both $\mathcal{T}^0$ and $\mathcal{T}^1$.
    \item (Challenge phase.) We choose a random bit $b \in \{0,1\}$ and run $\Pi$ with transaction tuple list $\mathcal{T}^b$
    \item $\mathcal{A}$ gets the flow output sent to each corrupted user from $\Pi$ as well as any updates to the internal state of the factory in the case where $\mathcal{A}$ corrupted some hub nodes.
    \item $\mathcal{A}$ outputs a bit $b'$. If $b'=b$, $\mathcal{A}$ wins the game.
\end{itemize}

We say a transaction aggregation and execution protocol $\Pi$ is $\epsilon$-private if $\mathcal{A}$ wins the above game with
probability at most $\frac{1}{2} + \epsilon$, and private if it is $\epsilon$-private for some negligible $\epsilon$.

\begin{comment}
\subsection{Examples}
In the following examples, the adversary corrupts the hubs in red. We first list example situations which should be indistinguishable to the adversary. 

\begin{enumerate}
    \item 
    \begin{minipage}[t]{\linewidth}
      (Adding transactions unrelated to corrupted hubs should be indistinguishable.) The factory consist of four hubs, $h_0, h_1, h_2, h_3$ and the adversary corrupts $h_0$. The two list of transaction tuples the adversary creates are $\mathcal{T}^0 = \{(1, A, B, h_0)\}$ and $\mathcal{T}^1 = \{(1, A, B, h_0), (1, C, D, h_2)\}$. \\ \newline                                
      \includegraphics[width=\textwidth]{./img/eg1.pdf}
    \end{minipage}\\
    
    \item 
    \begin{minipage}[t]{\linewidth}
      The factory consist of four hubs, $h_0, h_1, h_2, h_3$ and the adversary corrupts $h_1$ and $h_3$. The two list of transaction tuples the adversary creates are $\mathcal{T}^0 = \{(1,A,B,h_0), (1,C,D,h_2)\}$ and $\mathcal{T}^1 = \{(1, A, D, h_0), (1, C, B, h_2)\}$. \\ \newline                                
      \includegraphics[width=\textwidth]{./img/eg2.pdf}
    \end{minipage}\\
\end{enumerate}

Examples which are distinguishable:

\begin{enumerate}
    \item 
    \begin{minipage}[t]{\linewidth}
      The factory consist of four hubs, $h_0, h_1, h_2, h_3$ and the adversary corrupts $h_0$ and $h_2$. \\ \newline                                
      \includegraphics[width=\textwidth]{./img/simple_counter.pdf}
    \end{minipage}
\end{enumerate}
\end{comment}


